FlingBot: The Unreasonable Effectiveness of Dynamic Manipulation for Cloth Unfolding

High-velocity dynamic actions (e.g., fling or throw) play a crucial role in our everyday interaction with deformable objects by improving our efficiency and effectively expanding our physical reach range. Yet, most prior works have tackled cloth manipulation using exclusively single-arm quasi-static actions, which requires a large number of interactions for challenging initial cloth configurations and strictly limits the maximum cloth size by the robot's reach range. In this work, we demonstrate the effectiveness of dynamic flinging actions for cloth unfolding with our proposed self-supervised learning framework, FlingBot. Our approach learns how to unfold a piece of fabric from arbitrary initial configurations using a pick, stretch, and fling primitive for a dual-arm setup from visual observations. The final system achieves over 80% coverage within 3 actions on novel cloths, can unfold cloths larger than the system's reach range, and generalizes to T-shirts despite being trained on only rectangular cloths. We also finetuned FlingBot on a real-world dual-arm robot platform, where it increased the cloth coverage over 4 times more than the quasi-static baseline did. The simplicity of FlingBot combined with its superior performance over quasi-static baselines demonstrates the effectiveness of dynamic actions for deformable object manipulation.

==> text/spatial_action_maps_full.tex <==
To this end, we propose to learn a convolutional value network $V: \mathbb{R}^{H\times W\times 3} \rightarrow  \mathbb{R}^{H\times W}$ which is invariant to translation, rotation, and scale, which leads to grasp predictions equivariant to the cloth's transformations.
Given a visual observation $o\in \mathbb{R}^{H\times W\times 3}$ from the top-down camera view, we generate a batch of scaled and rotated observations $\{o_i\}$, then using $V$ to predict the corresponding batch of dense value maps $\{V(o_i)\}$.
Here, the value of each pixel $\langle x,y \rangle$ in each $V(o_i)$ corresponds to the predicted delta-coverage of executing the pick, stretch, and fling action parameterized by $\langle C_{x}=x,C_{y}=y, \theta=0, w=\bar{w}\rangle$ for some fixed $\bar{w}$ (e.g., 8 pixels).
While $\theta$ and $w$ are fixed constant to be 0 and $\bar{w}$ respectively in the transformed pixel space of $o_i$ for some rotation and scaling, we can apply the inverse rotation and scaling transformation to get varying grasp rotations and widths in the original pixel space of $o$.
By its architecture, $V$ is invariant to translation.
By rotating and scaling the inputs, $V$ is invariant to rotation and scale.

Hence, in this framework, each pixel in $V(o_i)$ corresponds to a unique and physically meaningful action.
At each time step, finding the next fling parameters amounts to evaluating $V(o_i)$ for $o_i$'s at different rotations and scaled grasp widths which satisfy the constraints of the system, then picking the parameterization corresponding to the pixel with the maximum value.
To apply this value network to the task of cloth-unfolding, we supervise $V$ to regress each pixel $\langle x,y\rangle$ in $V(o_i)$ to the delta-coverage of the fling action parameterized by $\langle C_{x},C_{y}, 0, \bar{w}\rangle$ by minimizing the $\mathcal{L}_2$ loss between the predicted and ground truth delta-coverage.
Thus, by picking the grasping action with the highest value, the system picks grasp points which lead to the greatest increase in the cloth coverage.


In our approach, we use 12 rotations, which discretizes the range $[-90^\circ,90^\circ]$, and $8$ scale factors in the range $[1.00,2.75]$ at $0.25$ intervals, with $\bar{w} = $ 8 pixels.
Our value network is a fully convolutional neural network with nine residual blocks~\cite{he2016deep} and two convolutional layers in the first and last layer, and takes as input $64\times 64$ RGB images.
To evaluate actions within a useful range of scales, we crop the image such that the cloth takes up at most two-thirds of the image width and height before further scaling it by the $8$ scale factors above.
We also filter out and reject all grasp point pairs which are out of reach for either arm.

